Towards Feature Space Adversarial Attack

We propose a new adversarial attack to Deep Neural Networks for image classification. Different from most existing attacks that directly perturb input pixels, our attack focuses on perturbing abstract features, more specifically, features that denote styles, including interpretable styles such as vivid colors and sharp outlines, and uninterpretable ones. It induces model misclassfication by injecting imperceptible style changes through an optimization procedure. We show that our attack can generate adversarial samples that are more natural-looking than the state-of-the-art unbounded attacks. The experiment also supports that existing pixel-space adversarial attack detection and defense techniques can hardly ensure robustness in the style related feature space.

==> attackspace.tex <==
We generate and visually analyze the two feature space attacks. The ImageNet model hardened by feature denoising is used for generating adversarial samples. Columns (a), (d), and (g) in \autoref{fig:images} (see \autoref{sec:appendix}) present the original images. Columns (b), (c), and (d) present the adversarial samples generate by the Encoder and the corresponding Decoder, with different encoder depths. Specifically, column (b) uses conv2\_1 layers, column (c) uses conv3\_1 layers and column (d) uses conv4\_1 layers of a pretrained VGG-19 as the Encoder, and the Decoders are of similar neural network structure with the corresponding Encoders in a reverse order. Observe that as the Encoder becomes  deeper, object outlines and textures are changed in addition to colors. 
Columns (e) and (f) are adversarial samples generated by the feature argumentation attack (FA) and feature interpolation attack (FI). We observe that they both generate realistic images.

%(h), (i) by the feature argumentation attack (FA).
%, respectively. 

%Columns (h) and (i) are adversarial samples by FA, restricting by only 
In column (h), we only perturb the mean of embedding whereas in column (i) we only perturb the standard deviation of embedding. The results indicate that mean values tend to represent the background and the overall color tone. In contrast, the standard deviations tend to represent the object shape and relative color. 

%Examples of feature augmentation space and feature interpolation space. We exhibit the successfully attacked images generated by this two space here.


%\begin{figure}[htp]
%\begin{subfigure}[b]{0.5\textwidth}
%    \centering
%    \includegraphics[height=10cm]{figures/fafi.png}
%    \caption{The adversarial samples of feature augmentation and feature interpolation. We choose the feature denoising model to generate adversarial samples. The images in column from left to right are respectively (a) normal images, (b)feature interpolation adversarial samples and (c) feature augmentation adversarial samples.  }
    
%    \label{fig:fafi}
%\end{subfigure}
%\begin{subfigure}[b]{0.5\textwidth}
%    \centering
%    \includegraphics[height=10cm]{figures/deeper.png}
%    \caption{The adversarial samples of feature augmentation from shallow to deep decoder. We use %certain layers of VGG-19 model as the encoder. Specifically column (a) use conv2\_1 layers, column %(b) use conv3\_1 layers and column (c) use conv4\_1 layers.   }
%    \label{fig:fafi}
%\end{subfigure}
%\end{figure}

%Here we show the adversarial samples gener encoder and decoder from shallow to deep by feature augmentation attack. 
%\begin{figure}[htp]

%\end{figure}
%And for each attack, attacker can change mean and variance independently. In this section, we compare intuitively what are their differences. Generally speaking, changing mean value of channel tends to change background and overall color. Changing standard deviation tends to change the object and relative color.

%\ql{display several images generated from shallow to high \\
%display several images generated by l\_2 linf and feature space attack }
